On Adversarial Robustness of Deep Image Deblurring

Recent approaches employ deep learning-based solutions for the recovery of a sharp image from its blurry observation. This paper introduces adversarial attacks against deep learning-based image deblurring methods and evaluates the robustness of these neural networks to untargeted and targeted attacks. We demonstrate that imperceptible distortion can significantly degrade the performance of state-of-the-art deblurring networks, even producing drastically different content in the output, indicating the strong need to include adversarially robust training not only in classification but also for image recovery.

==> fig_vary_eps.tex <==
\begin{figure*}[htb]
\begin{center}
%\hspace{-10pt}
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{c}


\hspace{-10pt}\begin{sideways}~~$\epsilon$=4/255\end{sideways}~\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/GAN_im2_adv_inp_eps4.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/GAN_im2_adv_pred_eps4.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/MPR_im2_adv_inp_eps4.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/MPR_im2_adv_pred_eps4.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/dpWiener_im2_adv_inp_eps4.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/dpWiener_im2_adv_pred_eps4.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/RGDN_im2_adv_inp_eps4.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/RGDN_im2_adv_pred_eps4.png}\\
\hspace{-10pt}\begin{sideways}~~$\epsilon$=8/255\end{sideways}~\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/GAN_im2_adv_inp_eps8.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/GAN_im2_adv_pred_eps8.png}

\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/MPR_im2_adv_inp_eps8.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/MPR_im2_adv_pred_eps8.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/dpWiener_im2_adv_inp_eps8.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/dpWiener_im2_adv_pred_eps8.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/RGDN_im2_adv_inp_eps8.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/RGDN_im2_adv_pred_eps8.png}\\

\hspace{-10pt}\begin{sideways}~~$\epsilon$=12/255\end{sideways}~\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/GAN_im2_adv_inp_eps12.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/GAN_im2_adv_pred_eps12.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/MPR_im2_adv_inp_eps12.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/MPR_im2_adv_pred_eps12.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/dpWiener_im2_adv_inp_eps12.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/dpWiener_im2_adv_pred_eps12.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/RGDN_im2_adv_inp_eps12.png}
\includegraphics[width=0.1\linewidth]{LaTeX/ims/vary_epsilon/RGDN_im2_adv_pred_eps12.png}\\
a)~DeblurGANv2\cite{kupyn2019deblurgan}~~~~~~~~~~~~~~~~~~~~~~~~~b)~MPRNet\cite{zamir2021multi}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~c)~Deep Wiener\cite{dong2020deep}~~~~~~~~~~~~~~~~~~~~~~d)~RGDN\cite{gong2020learning}\\
\end{tabular}}
\caption{Effect of strength of adversarial noise on targetted attacks for different networks. For each approach, the first column is the adversarial input and the second column is the network prediction.}\label{fig:vary_eps}
\end{center}
\end{figure*}

==> fig_vary_kernel_size.tex <==
\begin{figure}[htb]
\begin{center}
%\hspace{-10pt}
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{c}
\hspace{-10pt}\begin{sideways}~~Clean obs.\end{sideways}~\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/bim_ker25.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/bim_ker17.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/bim_ker11.png}\\

\hspace{-10pt}\begin{sideways}~~~~~~~~\cite{kupyn2019deblurgan}\end{sideways}~\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/GAN_adv_pred_eps4_ker25.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/GAN_adv_pred_eps4_ker17.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/GAN_adv_pred_eps4_ker11.png}\\

\hspace{-10pt}\begin{sideways}~~~~~~~~\cite{ zamir2021multi}\end{sideways}~\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/MPR_adv_pred_eps4_ker25.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/MPR_adv_pred_eps4_ker17.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/MPR_adv_pred_eps4_ker11.png}\\
\hspace{-10pt}\begin{sideways}~~~~~~~~\cite{dong2020deep}\end{sideways}~\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/dpWiener_adv_pred_eps4_ker25.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/dpWiener_adv_pred_eps4_ker17.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/dpWiener_adv_pred_eps4_ker11.png}\\

\hspace{-10pt}\begin{sideways}~~~~~~~~\cite{gong2020learning}\end{sideways}~\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/RGDN_adv_pred_eps4_ker25.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/RGDN_adv_pred_eps4_ker17.png}
\includegraphics[width=0.28\linewidth]{LaTeX/ims/vary_kernel/RGDN_adv_pred_eps4_ker11.png}\\
$k=25$~~~~~~~~~~~~~~~~~~~$k=17$~~~~~~~~~~~~~~~~$k=11$\\
\end{tabular}}
\caption{Effect of kernel size on ease of targetted attack for different deblurring networks for $\epsilon=4/255$.}\label{fig:vary_kernelsize}
\end{center}
\end{figure}

==> tabl_untargetted.tex <==
\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{ccccc}
\hline
     Network&clean&$\epsilon=4$&$\epsilon=8$&$\epsilon=12$\\
    \hline
    MPRNet~\cite{zamir2021multi}&24.78&&&\\
    DeblurGANv2~\cite{kupyn2019deblurgan}&\\
    Deep Wiener~\cite{dong2020deep}&\
    RGDN~\cite{gong2020learning}\\
    \hline
    \end{tabular}}
    \caption{Comparison of robustness to untargeted attacks.  Average PSNR values of the network predictions are reported for different strengths of adversarial noise. }
    \label{tab:untargetted}
\end{table}

